MedJev: Evaluating Zero-Shot System-One Decision Making in Medicine

System One decision models such as Jev answer structured questions in a single forward pass without generating text, offering fast and computationally efficient clinical decision support. We evaluate MedJev, an open System One model that runs locally on a laptop, across ten medical benchmarks spanning medical knowledge, diagnosis, and patient level prediction using MIMIC IV and MIMIC IV ED. We compare MedJev against zero shot LLM baselines, published GPT results, and supervised models. MedJev achieves accuracies of 72.5 percent on MedQA, 75.4 percent on USMLE, and 80.1 percent on NEJM, approaching published GPT 4 performance while maintaining well calibrated confidence estimates (ECE 0.028 to 0.063). On patient level tasks, MedJev achieves an AUROC of 0.926 for In Hospital Mortality, exceeding XGBoost (0.902), but underperforms supervised models on operational outcomes such as ED Triage Admission (0.745 vs. 0.809). Patient level predictions also exhibit substantial miscalibration (In Hospital Mortality ECE 0.286). We introduce a lightweight, two parameter recalibration method that adapts predictions to local patient populations using 50 to 200 labeled examples, reducing ECE to 0.007. Our findings establish open System One models as a promising zero shot baseline for medical AI, combining competitive predictive performance with low computational cost and efficient local calibration. We release our code and evaluation harness to support future research.

==> data/tab_datasets.tex <==
\begin{tabular}{lll}
\toprule
Benchmark & Question & Source \\
\midrule
MedQA & USMLE-style vignettes, 5 options & MedQA test (BigBio) \\
USMLE & USMLE-style vignettes, 4 options & MedQA-USMLE-4-options test \\
NEJM & Diagnostic vignettes released open-ended & NEJM-MedQA (Savage et al.) \\
DiagnosisArena & Published case reports, 4 diagnoses & DiagnosisArena \\
ED Triage Disposition & ED disposition at triage, 6 classes & MIMIC-IV-ED \\
\midrule
ED Triage Admission & Hospital admission, decided at triage & MIMIC-IV-ED \\
ED Admission at 2\,h & Hospital admission, 2\,h after ED arrival & MIMIC-IV (MEDS) \\
In-Hospital Mortality & In-hospital death, 24\,h after admission & MIMIC-IV (MEDS) \\
Length of Stay $>$ 7 Days & Stay $>$ 7 days, 24\,h after admission & MIMIC-IV (MEDS) \\
30-Day Readmission & Readmission within 30 days, at discharge & MIMIC-IV (MEDS) \\
\bottomrule
\end{tabular}


==> sections/abstract.tex <==
\begin{abstract}
System-One decision models such as Jev answer typed questions about a structured state (pick an option, estimate a
probability) in a single forward pass, without generating text. This makes them fast, cheap and calibratable, which
suits clinical decision support. We ask how far an open System-One model, MedJev, gets on medical decisions
\emph{zero-shot}, running locally on a laptop. We evaluate it on ten benchmarks cast as Jev requests. Four cover
knowledge and diagnosis (MedQA, USMLE, NEJM, DiagnosisArena). Six are patient-level decisions with leakage-safe cohorts from
MIMIC-IV (In-Hospital Mortality, Length of Stay $>$ 7 Days, 30-Day Readmission, ED Admission at 2\,h) and MIMIC-IV-ED (ED Triage Admission, ED Triage Disposition). We compare it with
zero-shot LLM baselines read out identically (its base model Qwen3.5-9B, the medical model MedGemma-1.5-4B and its general base Gemma-3-4B on the knowledge benchmarks, Qwen3.5-2B and
Pythia-2.8B), with GPT-3.5, GPT-4, GPT-4o and o1 results reported on the same benchmarks, and with XGBoost and TF-IDF models tuned on
1{,}000 local labels. Zero-shot, MedJev answers \resMedqaJevAcc\% of MedQA, \resUsmleJevAcc\% of USMLE and
\resNejmJevAcc\% of NEJM with well-calibrated confidence (ECE \resUsmleJevEce--\resNejmJevEce). That is within 2--4 points
of zero-shot GPT-4 as reported on the same MedQA questions (\resMedqaRefGptFour\% and \resUsmleRefGptFour\%), and far
above GPT-3.5 (\resMedqaRefGptThree\% and \resUsmleRefGptThree\%). It ranks In-Hospital Mortality risk with an AUROC of
\resMortalityJevAuroc, at least as well as supervised models with 1{,}000 labels (XGBoost \resMortalityXgbAuroc), and
matches them on 30-Day Readmission. It trails them on operational outcomes such as admission at triage (\resTriageJevAuroc{} vs.\
\resTriageXgbAuroc), where supervised models overtake it after about 100--200 local labels. Its patient-level
probabilities ignore local base rates (In-Hospital Mortality ECE \resMortalityJevEce); a two-parameter recalibration fitted on
50--200 local labels removes this (ECE \resMortalityPlattEce{} with 1{,}000). An open System-One model is thus a strong
zero-shot cold start for medical decisions, provided its probabilities are recalibrated locally. Code and evaluation
harness are released.
\end{abstract}


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

An open System-One model, used zero-shot, answers medical knowledge questions accurately and with calibrated
confidence, and ranks clinical severity as well as supervised models trained on 1{,}000 local cases. Its patient-level
probabilities do not reflect local base rates, but a two-parameter recalibration fitted on 50--200 local cases removes
that gap. Outcomes that depend on local operations remain where supervision pays off. The harness, benchmarks and
figures regenerate from cached model outputs, so new models and tasks can be compared under the same protocol.


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{What zero-shot System-One decisions do well.}
\emph{Knowledge without generation.} A 9B model answering in one forward pass, without chain-of-thought and on a
laptop, is accurate and well calibrated on USMLE-style questions: within a few points of zero-shot GPT-4 and far above
GPT-3.5 as reported on the same questions. Only an explicit reasoning model (o1) is reported ahead, on the hardest
benchmark (DiagnosisArena). Its confidence is usable for deferral as it stands (\cref{sec:res-sel}).
\emph{Ranking clinical severity without labels.} On In-Hospital Mortality, zero-shot MedJev ranks patients at least as well as
tuned supervised models trained on 1{,}000 local admissions, and on 30-Day Readmission none of them is significantly better. A hospital
without labelled data, or one that cannot share it, gets a usable risk ranking on day one.
\emph{The Jev training helps.} MedJev is ahead of its own base model on knowledge and on the severity outcomes, and
far better calibrated, under identical prompts and readout.

\paragraph{What it does not do.}
\emph{Calibrated risks on day one.} Zero-shot probabilities for patient-level outcomes ignore local base rates and
over-predict rare events (\cref{sec:res-cal}). Raw probabilities must not be used as risks or thresholded at 0.5.
Recalibration fixes this cheaply but needs in-domain labels: 50--200 local cases suffice, whereas a temperature carried
over from another benchmark does not help.
\emph{Operational outcomes.} Admission from the ED and long stays depend on how a hospital works (bed availability,
observation-unit policy, discharge planning) as much as on the clinical picture. Here supervised models overtake the
zero-shot ranking after roughly 100--200 local labels (\cref{sec:res-le}).
\emph{Rare options.} In a six-way \textsc{Choice} with rare options (transfer, expired), the zero-shot model almost never
chooses them, which keeps ED Triage Disposition accuracy below the supervised references.

\paragraph{Implications for a medical System-One model.}
A deployable MedJev can start zero-shot and become locally calibrated within its first few hundred labelled cases, with
a calibration map that is monotone, has two parameters and is easy to audit and monitor. For outcomes driven by local
operations, a supervised model trained on a few hundred local cases remains the stronger choice. The zero-shot model is
then the right cold-start and fallback.

\paragraph{Limitations.}
\begin{itemize}[leftmargin=*, itemsep=1pt]
  % NOTE (not printed): for compute, each benchmark is evaluated on a random sample of up to 1,000 test examples
  % (one per patient for EHR benchmarks), and the supervised references use up to 1,000 training labels.
  \item \emph{Sample sizes.} At
        natural prevalence, In-Hospital Mortality has only \resMortalityPos{} test deaths, so its AUROC and AUPRC carry wide intervals.
  \item \emph{One prompt, one serialisation.} Questions, state layouts and list caps were fixed in advance and not tuned.
        Both are known to matter for LLM classifiers on serialised data \citep{hegselmann2023tabllm}.
  \item \emph{Format mismatch.} NEJM was released open-ended. We score it as multiple choice, so the published GPT
        accuracies are a reference point, not a like-for-like comparison.
  \item \emph{Overlap and contamination.} MedQA and USMLE share their question stems, and MedQA has been public since
        2020, so it may be in the models' pretraining data.
  \item \emph{Incomplete code vocabulary.} The MEDS extract ships no ICU item dictionary. Bedside measurements are named
        from standard MIMIC-IV item identifiers, and other chart events are omitted from the states.
  \item \emph{Single site.} MIMIC-IV and MIMIC-IV-ED come from one academic medical centre.
\end{itemize}

\paragraph{Data use and ethics.}
MIMIC-IV and MIMIC-IV-ED were accessed under the PhysioNet credentialed data use agreement. All processing and inference
ran locally, the model server was bound to the loopback interface, and no individual-level data appear in this paper.
Calibration maps fitted on these data are not released publicly. The models evaluated here are research artefacts and
must not be used for clinical decisions.


==> sections/experiments.tex <==
\section{Experimental Setup}
\label{sec:setup}

\begin{table}[t]
  \centering
  \caption{The ten benchmarks. Top: knowledge and diagnosis (\textsc{Choice}). Bottom: patient-level decisions from
  EHRs (\textsc{Noul}, except the six-way ED Triage Disposition).}
  \label{tab:datasets}
  \small
  \resizebox{\linewidth}{!}{\input{generated/tab_datasets}}
\end{table}

\begin{table}[t]
  \centering
  \caption{Full statistics of the ten benchmarks. Train, validation and test are the benchmarks' own splits; for the
  EHR benchmarks they are the MEDS \texttt{train}, \texttt{tuning} and \texttt{held\_out} patient splits, and every unit
  (admission, ED visit or ED stay) meets the cohort definition of \cref{sec:tasks}. \emph{Patients}: distinct patients
  over all splits. \emph{Label balance}: share of each answer letter on the test split (knowledge benchmarks), share of
  each disposition (ED Triage Disposition) or prevalence over all splits (binary benchmarks).}
  \label{tab:stats}
  \small
  \resizebox{\linewidth}{!}{\input{generated/tab_stats}}
\end{table}

\paragraph{Data.}
\Cref{tab:stats} gives the full size and label balance of every benchmark. The MEDS benchmarks use a MEDS-Transforms extract \citep{medstransforms} of MIMIC-IV v2.2 (299{,}712 patients in five
\texttt{train}, one \texttt{tuning} and one \texttt{held\_out} shard). Test patients come from \texttt{held\_out} and
training patients from \texttt{train}. MIMIC-IV-ED v2.2 contributes 425{,}087 ED stays; we keep adults with a MEDS birth
record and assign each patient to the MEDS split of the same \texttt{subject\_id}.

\paragraph{Models and serving.}
All language models run locally on one Apple silicon laptop (48\,GB unified memory) through MLX \citep{mlx2023}, in
8-bit builds. A local engine loads the frozen MedJev helper and replaces only its model client. Its answers match the
MedJev HTTP server's exactly on a verification sample (maximum absolute probability difference 0). MedJev answers a
MedQA question in about 0.5\,s and a MEDS state in about 2\,s. No patient data leave the machine.


==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

Most uses of language models in medicine are \emph{generative}: a model writes an answer or a rationale, and a person or
a parser extracts the decision \citep{singhal2023medpalm}. Many clinical workflows need the decision itself: whether to
request a bed at triage, whether a patient is at risk of dying in hospital, whether a stay will be long. For such
decisions the useful output is a calibrated probability over a fixed set of options. It should be produced quickly and
cheaply, and in a form that can be thresholded, audited and monitored.

\emph{System-One} models, named after the fast mode of human judgment \citep{kahneman2011thinking}, are built for this.
TypeSafe's Jev \citep{typesafe2026jev} takes a \emph{state} (text or JSON) and typed \emph{questions}: a \textsc{Choice}
over named options, a \textsc{Noul} (the probability that a statement is true) or a \textsc{Score} on an ordinal scale.
Each is answered with a full distribution from one prefill, without generation. An independent benchmark of Jev on 37
public datasets found competitive zero-shot accuracy at very low cost \citep{deusser2026jev}, but it did not cover
medicine. Jev is also closed and hosted, so credentialed patient data cannot be sent to it.

This paper asks how far an open System-One model gets on medical decisions \emph{zero-shot}, with no task data at all.
We study OpenJev Flash 9B \citep{openjev2026flash}, an open-weight model that implements the Jev interface and runs on a
laptop, and compare it on equal footing with three groups of references. We call it \emph{MedJev} when it is used zero-shot on medical Jev requests, as throughout this paper. The first is zero-shot language models read out identically: its own base model, an open medical model (MedGemma) and its general base (Gemma), a smaller model from the same
family, and a base model without instruction tuning. The second is frontier models (GPT-3.5, GPT-4, GPT-4o, o1) as
reported by other studies on the same benchmarks. The third is
supervised models trained on 1{,}000 local labels per task. We also ask what a hospital would have to add before
trusting the zero-shot probabilities, and how many local labels a supervised model needs to catch up.

\paragraph{Contributions.}
\begin{enumerate}[leftmargin=*, itemsep=2pt]
  \item Ten medical benchmarks in the Jev request format, each with one short name. Four test knowledge and diagnosis
        (MedQA, USMLE, NEJM, DiagnosisArena). Six test patient-level decisions from raw EHR data, with explicit, leakage-safe
        cohorts and prediction times: In-Hospital Mortality, Length of Stay $>$ 7 Days, 30-Day Readmission and ED Admission at 2\,h from MIMIC-IV in MEDS, and ED Triage Admission
        and ED Triage Disposition from MIMIC-IV-ED (\cref{sec:tasks}).
  \item A controlled zero-shot evaluation. MedJev is compared with zero-shot LLM baselines under identical prompts and
        readout, and with tuned supervised references capped at 1{,}000 labels. All models are scored on identical test
        examples with paired tests (\cref{sec:variants,sec:fairness}).
  \item Evidence on where zero-shot System-One decisions work and where they need help. They are accurate and
        calibrated on medical knowledge, within a few points of zero-shot GPT-4 on MedQA, and they rank clinical severity as well as supervised models with 1{,}000 labels.
        Their patient-level probabilities, however, ignore local base rates, which two-parameter recalibration on 50--200
        local labels corrects (\cref{sec:results}).
  \item An open harness that caches every model output, so new models, tasks and analyses can be added without
        re-querying the model.
\end{enumerate}


==> sections/method.tex <==
\section{Method}
\label{sec:method}

\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
      font=\small,
      box/.style={draw=jevblue, rounded corners=2pt, thick, align=center, minimum height=0.95cm, inner sep=3pt, fill=jevblue!6},
      data/.style={draw=jevgrey, rounded corners=2pt, align=center, minimum height=0.95cm, inner sep=3pt, fill=jevgrey!10},
      arr/.style={-{Stealth[length=2.0mm]}, thick, draw=jevgrey!80!black}]
    \node[data, text width=2.7cm] (qa) {Knowledge QA\\\scriptsize MedQA, USMLE, NEJM, DiagnosisArena};
    \node[data, text width=2.7cm, below=0.35cm of qa] (ehr) {EHR event streams\\\scriptsize MIMIC-IV (MEDS)};
    \node[data, text width=2.7cm, below=0.35cm of ehr] (ed) {ED triage records\\\scriptsize MIMIC-IV-ED};
    \node[box, right=0.6cm of ehr, text width=2.4cm] (req) {Jev request\\\scriptsize state + \textsc{Choice}/\textsc{Noul}};
    \node[box, right=0.6cm of req, text width=2.7cm, fill=jevblue!14] (jev) {MedJev\\\scriptsize zero-shot, 1 prefill};
    \node[box, right=0.6cm of jev, text width=2.6cm] (cal) {optional local\\recalibration\\\scriptsize monotone, 2 parameters};
    \draw[arr] (qa.east) -- (req.west);
    \draw[arr] (ehr.east) -- (req.west);
    \draw[arr] (ed.east) -- (req.west);
    \draw[arr] (req) -- (jev);
    \draw[arr] (jev) -- (cal);
  \end{tikzpicture}
  \caption{Open MedJev. Each benchmark becomes Jev requests (a state plus typed questions), which MedJev answers
  zero-shot. An optional two-parameter recalibration maps its probabilities onto local base rates without changing its
  ranking. Zero-shot LLM baselines and label-capped supervised references are scored on the same test examples.}
  \label{fig:pipeline}
\end{figure}

\subsection{The Jev request format and the MedJev readout}
\label{sec:jev}

A Jev request is a pair $(s, Q)$ of a state $s$ (text or JSON) and a map of questions $Q$. A \textsc{Choice} question
has instructions and $K$ named options and returns a distribution over them. A \textsc{Noul} question has instructions
and optional descriptions of the true and false outcomes, and returns $p_{\text{yes}} \in [0,1]$. MedJev (OpenJev Flash 9B,
\citealp{openjev2026flash}) renders each question as one chat prompt (state, instructions, options labelled with
single-token letters), then reads the logits $\ell_1,\dots,\ell_K$ of the letter tokens at the first answer position:
\begin{equation}
  p_i = \frac{\exp(\ell_i / T)}{\sum_{j=1}^{K} \exp(\ell_j / T)}.
  \label{eq:readout}
\end{equation}
A \textsc{Noul} is a two-option readout (yes/no) followed by
\begin{equation}
  p_{\text{yes}} = \sigma\!\left(\frac{1}{T_{\text{N}}}\log\frac{p_1}{1-p_1} + b\right).
  \label{eq:noul}
\end{equation}
We use the published settings of the MLX build ($T=1.07$, $T_{\text{N}}=1.0748$, $b=0$) and the frozen helper code that
implements them (SHA-256 prefix \texttt{81a22f1b}). The zero-shot LLM baselines use the same helper, so every language
model sees identical prompts and is read out identically.

\subsection{Benchmarks}
\label{sec:tasks}

\Cref{tab:datasets} lists the ten benchmarks. Each has one short name, which is used throughout the paper.

\paragraph{Knowledge and diagnosis (\textsc{Choice}).}
\emph{MedQA} and \emph{USMLE} are the five-option (BigBio) and four-option (MedQA-USMLE-4-options) releases of the
USMLE-style MedQA questions \citep{jin2021medqa}. \emph{DiagnosisArena} (DiagnosisArena, \citealp{zhu2025diagnosisarena}) holds
915 published case reports (history, examination, tests) with four candidate final diagnoses. \emph{NEJM} (NEJM-MedQA,
\citealp{savage2024diagnostic}) holds 512 diagnostic vignettes that were released \emph{open-ended}, together with
free-text GPT-3.5 and GPT-4 answers graded by clinicians under several reasoning prompts. Jev cannot generate, so we
pose every vignette as a \textsc{Choice}. Vignettes found in MedQA keep their five MedQA options; the rest receive the
gold diagnosis, up to four GPT answers that were graded wrong, and other vignettes' diagnoses as padding. Our format is
easier than the open-ended one, so the published GPT accuracies are a reference point, not a like-for-like comparison.

\paragraph{Patient-level prediction from EHR event streams (\textsc{Noul}).}
MIMIC-IV \citep{johnson2023mimiciv} in the MEDS format \citep{arnrich2024meds} stores each patient as time-stamped coded
events and carries no labels. We define four cohorts with a fixed prediction time $t^\ast$. \emph{In-Hospital Mortality}
(in-hospital death) and \emph{Length of Stay $>$ 7 Days} (a stay longer than 7 days) cover adults still in hospital at
$t^\ast = t_{\text{adm}} + 24$\,h. \emph{30-Day Readmission} is a new admission within 30 days, predicted at discharge.
\emph{ED Admission at 2\,h} is hospital admission, predicted 2\,h after emergency-department arrival. Only events in
$(t^\ast - 365\,\text{d}, t^\ast]$ are visible. Diagnoses and DRGs are stamped at discharge in MEDS, so they cannot
leak into the 24\,h benchmarks. For ED Admission at 2\,h, every field that exists only for admitted patients is withheld: race,
insurance, language and marital status live on admission rows; ED and admission bookkeeping codes from 24\,h before
arrival onward are dropped; and after arrival only laboratory events are kept. Each window is rendered as a compact JSON
state.

\paragraph{Emergency-department triage (MIMIC-IV-ED).}
At triage the decision is least informed and most useful for patient flow \citep{hong2018triage}. The state holds only
what triage records (\cref{fig:state}): arrival transport, sex, race, age, the triage vital signs, pain, acuity (ESI)
and chief complaint, plus past-year ED history from earlier stays \citep{johnson2023mimicived}. Medications, later
vitals, medication reconciliation (charted a median 69\,min after arrival) and diagnoses are excluded.
\emph{ED Triage Admission} asks whether the patient will be admitted (\textsc{Noul}). \emph{ED Triage Disposition} asks for the
disposition among six options: home, admitted, transfer, left before completion, expired or other (\textsc{Choice}).

\begin{figure}[t]
\begin{lstlisting}
{"decision_time": "at emergency department triage",
 "patient": {"age": 67, "sex": "male", "race": "WHITE"}, "arrival_transport": "AMBULANCE",
 "triage": {"temperature_F": 100.9, "heart_rate_bpm": 118, "respiratory_rate": 24, "o2_saturation_pct": 91,
            "systolic_bp_mmHg": 96, "diastolic_bp_mmHg": 58, "pain": "4", "acuity_esi": 2, "chief_complaint": "Dyspnea"},
 "past_year_emergency_department_history": {"visits": 3, "visits_ending_in_admission": 2}}
Question (Noul): Based on the information available at emergency department triage, will this visit end with the
patient admitted to the hospital?
\end{lstlisting}
\caption{An illustrative (synthetic) ED Triage Admission state and its \textsc{Noul} question. No real patient data are shown,
in accordance with the MIMIC data use agreements. MEDS states have the same structure, with demographics, prior-year
history, care units, latest laboratory values (flagged high/low at $|z|>2$) and medications.}
\label{fig:state}
\end{figure}

\subsection{Models compared}
\label{sec:variants}

\begin{description}[leftmargin=0pt, itemsep=2pt]
  \item[MedJev, zero-shot.] The readout of \cref{eq:readout,eq:noul}, with no task data of any kind.
  \item[MedJev + recalibration.] The only local step we allow the zero-shot model: Platt scaling
    \citep{platt1999probabilistic} of its \textsc{Noul} logit, or temperature scaling \citep{guo2017calibration} of its
    \textsc{Choice} distribution, fitted on its own zero-shot answers to labelled training examples. Both maps are
    monotone with at most two parameters. They change the probability scale but leave the ranking intact, and they can be
    audited at a glance. The QA benchmarks share one temperature fitted on MedQA training questions.
  \item[Zero-shot LLM baselines.] Qwen3.5-9B, the base model that MedJev was fine-tuned from \citep{qwen2026qwen35},
    isolates what the Jev training contributes. Qwen3.5-2B, a smaller model from the same family, shows the effect of
    scale. Both use exactly MedJev's prompts and readout. On the knowledge benchmarks we add MedGemma-1.5-4B
    \citep{sellergren2025medgemma}, Google's open medical model (Gemma~3, instruction-tuned on medical text and images;
    text only here), and Gemma-3-4B \citep{gemma2025gemma3}, the general model it is built on, both with the same prompts
    and their own chat template and option-letter tokens. Comparing the two isolates the effect of medical training. Pythia-2.8B \citep{biderman2023pythia}, a base language model
    without instruction tuning or a chat template, receives the same rendered prompt followed by ``Answer:'' and is read
    out from its own option-letter tokens; its 2{,}048-token context truncates the longest EHR prompts from the left,
    which keeps the question and options.
  \item[Published references.] Accuracies reported by other studies on the same test questions, without re-running
    them: zero-shot GPT-4 and GPT-3.5 on the MedQA US test set in its 5-option (MedQA) and 4-option (USMLE) forms
    \citep[Table~5]{nori2023capabilities}; the best clinician-graded \emph{open-ended} accuracy of GPT-4 and GPT-3.5
    across reasoning prompts on NEJM \citep{savage2024diagnostic}; and the multiple-choice accuracy of GPT-4o and of the
    reasoning model o1 on DiagnosisArena \citep{zhu2025diagnosisarena}. These numbers come from different prompts and, for
    DiagnosisArena, from the full 1{,}113-case benchmark, of which the public release we use has 915 cases. They are therefore
    reference points, not paired comparisons.
  \item[Supervised references (EHR benchmarks only).] Models trained on local labelled examples from each benchmark's
    training split and tuned as well as the labels allow. XGBoost \citep{chen2016xgboost} uses bag-of-codes features for MEDS (per-code counts and
    last values) and, for triage, structured triage fields plus chief-complaint tokens, the standard tabular approach
    \citep{hong2018triage}. TF-IDF with logistic regression uses the serialised state. Tree depth, column subsampling,
    child weight and the number of trees (XGBoost), and the $n$-gram range and regularisation (TF-IDF), are chosen by
    five-fold cross-validation on the training examples; the model is then refit on all of them.
\end{description}

\subsection{Evaluation protocol}
\label{sec:fairness}

Every model is scored on the same test examples. Every model that learns from labels (recalibration, XGBoost, TF-IDF)
sees the same labelled training examples, from training splits that share no patient with the test sets: MEDS train
patients, and MIMIC-IV-ED patients in the MEDS train split. Hyperparameters are chosen without test data, and
\cref{sec:res-le} studies how performance depends on the number of local labels. Differences against zero-shot MedJev are tested with paired
bootstraps over test examples. For \textsc{Choice} benchmarks we report accuracy and the ECE (15 equal-width bins,
\citealp{guo2017calibration}) of the top-option probability. For \textsc{Noul} benchmarks we report AUROC, AUPRC, ECE and
Brier score. Confidence intervals are 95\% percentile bootstrap intervals over test examples \citep{efron1993bootstrap}.


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{System-One decision models.}
Jev \citep{typesafe2026jev} exposes \textsc{Choice}, \textsc{Noul} and \textsc{Score} primitives over a state and returns
probabilities instead of text. \citet{deusser2026jev} benchmark it zero-shot on 37 public datasets and compare it with
open-weight LLMs scored through exact option probabilities. Their suite includes one biomedical dataset (PubMedQA,
\citealp{jin2019pubmedqa}) and no EHR prediction. OpenJev \citep{openjev2026flash} re-implements the interface by
fine-tuning Qwen3.5-9B \citep{qwen2026qwen35} and reads answers from the letter-token distribution after temperature
calibration. We use it, zero-shot and unchanged, as MedJev.

\paragraph{Medical question answering and diagnosis.}
MedQA \citep{jin2021medqa}, MedMCQA \citep{pal2022medmcqa} and PubMedQA \citep{jin2019pubmedqa} probe medical knowledge,
and large generative models exceed passing scores on USMLE-style questions \citep{singhal2023medpalm}. DiagnosisArena
\citep{zhu2025diagnosisarena} uses published case reports for harder differential diagnosis. \citet{savage2024diagnostic}
grade open-ended GPT-3.5 and GPT-4 diagnoses on MedQA vignettes under several reasoning prompts.

\paragraph{Clinical prediction from EHRs.}
In-hospital mortality, length of stay and readmission are long-standing MIMIC benchmarks
\citep{johnson2023mimiciv,harutyunyan2019benchmark}. MEDS \citep{arnrich2024meds} standardises patients as coded event
streams. Admission prediction at ED triage is a classic tabular task, in which gradient boosting on triage fields and
chief complaints is the standard approach \citep{hong2018triage}. Serialising ED records as text enables language
models on these tasks \citep{lee2024meme}. Few-shot evaluation of foundation models on structured EHRs is studied by
EHRSHOT \citep{wornow2023ehrshot}.

\paragraph{Language models on serialised data, and calibration.}
TabLLM \citep{hegselmann2023tabllm} classifies serialised table rows with an LLM: strong with few labels, weaker than
gradient-boosted trees with many. Tree ensembles remain strong on tabular data \citep{grinsztajn2022tree}. Post-hoc
recalibration (Platt scaling, temperature scaling; \citealp{platt1999probabilistic,guo2017calibration}) corrects
probability scales without changing rankings. We use it as the one local step on top of a zero-shot model.


==> sections/results.tex <==
\section{Results}
\label{sec:results}

\Cref{tab:mc,tab:binary} give every model on every benchmark, and \cref{tab:delta} tests each against zero-shot
MedJev on the same examples. Four findings stand out. Zero-shot MedJev is a strong, calibrated knowledge model
(\cref{sec:res-qa}). It ranks clinical severity as well as supervised models with 1{,}000 labels, but trails them on
operational outcomes (\cref{sec:res-ehr}). Its patient-level probabilities need local recalibration, which is cheap
(\cref{sec:res-cal}). And a supervised model needs from about a hundred to more than a thousand local labels to catch
up with its ranking (\cref{sec:res-le}).

\begin{table}[t]
  \centering
  \caption{Multiple-choice benchmarks: accuracy (\%) and, in parentheses, ECE. Supervised references apply only to
  the EHR benchmark ED Triage Disposition. Bottom: accuracies reported by other studies (\cref{sec:variants}); $^\dagger$ open-ended
  answers, a harder format.}
  \label{tab:mc}
  \small
  \resizebox{\linewidth}{!}{\input{generated/tab_mc}}
\end{table}

\begin{table}[t]
  \centering
  \caption{Binary EHR benchmarks: AUROC and, in parentheses, ECE. Recalibration is monotone, so it leaves AUROC
  unchanged and only moves ECE.}
  \label{tab:binary}
  \small
  \resizebox{\linewidth}{!}{\input{generated/tab_binary}}
\end{table}

\subsection{Medical knowledge and diagnosis}
\label{sec:res-qa}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_mc_accuracy}
  \caption{Accuracy on the multiple-choice benchmarks with 95\% bootstrap CIs; grey bars mark chance. Black and dark
  grey markers are accuracies reported by other studies on the same questions: zero-shot GPT-4 and GPT-3.5 on MedQA and
  USMLE \citep{nori2023capabilities}, their best open-ended accuracy on NEJM \citep{savage2024diagnostic}, and GPT-4o and
  o1 on DiagnosisArena \citep{zhu2025diagnosisarena}.}
  \label{fig:mc}
\end{figure}

Zero-shot, MedJev answers \resMedqaJevAcc\% of MedQA (95\% CI \resMedqaJevAccCI), \resUsmleJevAcc\% of USMLE
(\resUsmleJevAccCI), \resNejmJevAcc\% of NEJM (\resNejmJevAccCI) and \resDiagarenaJevAcc\% of DiagnosisArena
(\resDiagarenaJevAccCI), against chance rates of 20--25\% (\cref{fig:mc}). The Jev training is responsible for part of
this: under identical prompts and readout, its base model Qwen3.5-9B differs by \resMedqaBaseDelta{} and \resUsmleBaseDelta{}
points on MedQA and USMLE (paired CIs \resMedqaBaseDeltaCI{} and \resUsmleBaseDeltaCI), with smaller,
non-significant gaps on NEJM (\resNejmBaseDelta) and DiagnosisArena (\resDiagarenaBaseDelta). Scale matters more:
Qwen3.5-2B reaches only \resMedqaSmallAcc\%, \resUsmleSmallAcc\%, \resNejmSmallAcc\% and \resDiagarenaSmallAcc\%. Instruction
tuning matters most: Pythia-2.8B, a base language model, is at chance on all four (\resMedqaPythiaAcc\%,
\resUsmlePythiaAcc\%, \resNejmPythiaAcc\% and \resDiagarenaPythiaAcc\%), so the Jev format by itself does not supply the
knowledge. Domain specialisation does not close the gap at small scale either: MedGemma-1.5-4B, an open medical model,
reaches \resMedqaMedgemmaAcc\%, \resUsmleMedgemmaAcc\%, \resNejmMedgemmaAcc\% and \resDiagarenaMedgemmaAcc\%. That is
above Qwen3.5-2B but 13--25 points below MedJev (paired differences \resMedqaMedgemmaDelta{} to
\resDiagarenaMedgemmaDelta), and it is the least calibrated model on these benchmarks (ECE \resNejmMedgemmaEce--%
\resDiagarenaMedgemmaEce). Our single-token readout without reasoning may understate it relative to its developers' own
prompting, but the same readout serves MedJev well. Medical training itself does help at this scale. Its general base
model Gemma-3-4B reaches only \resMedqaGemmaAcc\%, \resUsmleGemmaAcc\%, \resNejmGemmaAcc\% and \resDiagarenaGemmaAcc\%, so
MedGemma gains 6--20 points, and it roughly halves Gemma's calibration error (Gemma ECE \resUsmleGemmaEce--%
\resDiagarenaGemmaEce, the most overconfident model in our study). 

\emph{Against reported frontier models.} On the same MedQA test questions, zero-shot GPT-4 is reported at
\resMedqaRefGptFour\% (5 options) and \resUsmleRefGptFour\% (4 options), and zero-shot GPT-3.5 at \resMedqaRefGptThree\%
and \resUsmleRefGptThree\% \citep{nori2023capabilities}. Zero-shot MedJev, a 9B model answering in one forward pass on
a laptop, is therefore within 2--4 points of zero-shot GPT-4 and almost 30 points above GPT-3.5. On NEJM, MedJev's
\resNejmJevAcc\% exceeds the best open-ended accuracy of GPT-4 across reasoning prompts (\resNejmGptFourMin--%
\resNejmGptFourMax\%; GPT-3.5 \resNejmGptThreeMin--\resNejmGptThreeMax\%; \citealp{savage2024diagnostic}). That format
is harder, so the comparison bounds rather than settles the question. DiagnosisArena, built from published case reports with
closely related candidate diagnoses, is the hardest benchmark for every model. There MedJev's \resDiagarenaJevAcc\% is
above the reported multiple-choice accuracy of GPT-4o (\resDiagarenaRefGptFourO\%) and below that of the reasoning model
o1 (\resDiagarenaRefOone\%) \citep{zhu2025diagnosisarena}, on a 915-case public subset of their benchmark.

\subsection{Patient-level decisions from EHRs}
\label{sec:res-ehr}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_binary_auroc}
  \caption{AUROC on the binary EHR benchmarks with 95\% bootstrap CIs. Zero-shot models use no labels; supervised
  references are trained on local labels with cross-validated hyperparameters. All models score the same test examples.}
  \label{fig:auroc}
\end{figure}

\begin{table}[t]
  \centering
  \caption{Paired differences against zero-shot MedJev on identical test examples (AUROC for binary benchmarks,
  accuracy points for multiple choice), with 95\% paired bootstrap CIs. Negative values favour MedJev.}
  \label{tab:delta}
  \small
  \resizebox{\linewidth}{!}{\input{generated/tab_delta}}
\end{table}

The EHR benchmarks split into two groups (\cref{fig:auroc,tab:delta}).

\emph{Clinical severity: zero-shot is as good as supervised.} On In-Hospital Mortality, zero-shot MedJev reaches an AUROC of
\resMortalityJevAuroc{} (CI \resMortalityJevAurocCI). Tuned XGBoost with 1{,}000 labelled admissions reaches
\resMortalityXgbAuroc{} (paired difference \resMortalityXgbDelta, CI \resMortalityXgbDeltaCI), and TF-IDF
\resMortalityTfidfAuroc{} (\resMortalityTfidfDelta, CI \resMortalityTfidfDeltaCI). On 30-Day Readmission, MedJev, its base model and the supervised
references all lie between 0.65 and 0.69, and no supervised model is significantly better than zero-shot MedJev (XGBoost
\resReadmissionXgbDelta, CI \resReadmissionXgbDeltaCI).

\emph{Operational outcomes: supervision wins.} Whether an ED visit ends in admission depends on local practice as much
as on the patient. Here XGBoost is ahead by \resTriageXgbDelta{} at triage (CI \resTriageXgbDeltaCI) and by
\resEdmedsXgbDelta{} at 2\,h (CI \resEdmedsXgbDeltaCI), and on ED Triage Disposition it is \resTriageDispXgbDelta{} accuracy points
ahead (CI \resTriageDispXgbDeltaCI). On Length of Stay $>$ 7 Days, TF-IDF is ahead by \resLongLOSTfidfDelta{} (CI \resLongLOSTfidfDeltaCI).

Among zero-shot models, MedJev beats its base model on the severity outcomes (In-Hospital Mortality \resMortalityBaseDelta,
Length of Stay $>$ 7 Days \resLongLOSBaseDelta), whereas on ED admission the base model is slightly ahead (\resEdmedsBaseDelta{} at
2\,h). Qwen3.5-2B is far behind on every EHR benchmark (e.g.\ In-Hospital Mortality \resMortalitySmallAuroc), is at chance on 30-Day Readmission
(\resReadmissionSmallAuroc) and ranks Length of Stay $>$ 7 Days below chance (\resLongLOSSmallAuroc): reading a long serialised patient
record is beyond a 2B model. Pythia-2.8B keeps some signal on the severity outcomes (In-Hospital Mortality \resMortalityPythiaAuroc,
Length of Stay $>$ 7 Days \resLongLOSPythiaAuroc) but none at triage (ED Triage Admission \resTriagePythiaAuroc), and on ED Triage Disposition it almost
always picks a wrong, rare option (\resTriageDispPythiaAcc\% accuracy).

\subsection{Calibration and recalibration}
\label{sec:res-cal}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_ece}
  \caption{Expected calibration error per benchmark for zero-shot MedJev, MedJev after recalibration, its base model
  and XGBoost (lower is better).}
  \label{fig:ece}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_calibration_curves}
  \caption{Calibration curves (prediction deciles; the dashed diagonal is perfect calibration). Multiple-choice panels
  plot accuracy against the top-option probability; binary panels plot the observed event rate against the predicted
  probability.}
  \label{fig:calcurves}
\end{figure}

On knowledge questions, zero-shot MedJev is well calibrated: ECE is \resMedqaJevEce{} on MedQA, \resUsmleJevEce{} on
USMLE and \resNejmJevEce{} on NEJM (\cref{fig:ece,fig:calcurves}). On patient-level questions it is not, because it
cannot know local base rates. The mean predicted probability of death is \resMortalityJevMeanProb{} against an observed
\resMortalityPrev\% (ECE \resMortalityJevEce), and ECE is \resLongLOSJevEce{} for Length of Stay $>$ 7 Days, \resReadmissionJevEce{} for
30-Day Readmission and \resTriageJevEce{} for ED Triage Admission. Recalibration on the training answers fixes this without touching the
ranking. ECE falls to \resMortalityPlattEce, \resLongLOSPlattEce, \resReadmissionPlattEce{} and \resTriagePlattEce{},
on par with or below XGBoost (\resMortalityXgbEce, \resLongLOSXgbEce, \resReadmissionXgbEce, \resTriageXgbEce). The Jev
training itself improves calibration substantially: the base model's zero-shot ECE is \resMortalityBaseEce,
\resLongLOSBaseEce{} and \resReadmissionBaseEce{} on the same benchmarks.

Recalibration needs in-domain data. A temperature fitted on MedQA training questions does not improve USMLE
(\resUsmleJevEce{} to \resUsmlePlattEce) or NEJM (\resNejmJevEce{} to \resNejmPlattEce), and it worsens DiagnosisArena
(\resDiagarenaJevEce{} to \resDiagarenaPlattEce), whose case reports are harder than USMLE vignettes.

\subsection{How many labels does supervision need to catch up?}
\label{sec:res-le}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_label_efficiency}
  \caption{Label efficiency, from cached outputs (no extra model queries). Top: ECE of recalibrated MedJev against the
  number of local labels. Bottom: AUROC of the supervised references trained on that many labels. Dashed: zero-shot
  MedJev (no labels). Mean $\pm$ s.d.\ over 10 random draws per budget.}
  \label{fig:le}
\end{figure}

\Cref{fig:le} varies the label budget from 25 to 1{,}000. Recalibration is cheap: with 50 labels Platt scaling cuts
In-Hospital Mortality ECE from \resMortalityJevEce{} to about 0.03, and with 200 labels ECE is between 0.014 and 0.064 on every
benchmark. Matching the zero-shot ranking with a supervised model is expensive and benchmark-dependent. XGBoost needs
about 100 labels on ED Admission at 2\,h and about 200 on ED Triage Admission, and TF-IDF needs about 200 on Length of Stay $>$ 7 Days. On 30-Day Readmission roughly
1{,}000 labels are needed, and on In-Hospital Mortality neither model reaches zero-shot MedJev even with 1{,}000.

\subsection{Selective prediction}
\label{sec:res-sel}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_selective}
  \caption{Accuracy among the answered questions when only the most confident fraction (coverage) is answered.}
  \label{fig:selective}
\end{figure}

A System-One answer carries its own confidence, so a deployment can answer confident cases and defer the rest
(\cref{fig:selective}). On the knowledge benchmarks, zero-shot MedJev's accuracy rises steadily as coverage shrinks,
consistent with its calibration there, and it stays above the base model's at almost every coverage.

